A Survey among Network Operators on BGP Prefix Hijacking

BGP prefix hijacking is a threat to Internet operators and users. Several mechanisms or modifications to BGP that protect the Internet against it have been proposed. However, the reality is that most operators have not deployed them and are reluctant to do so in the near future. Instead, they rely on basic - and often inefficient - proactive defenses to reduce the impact of hijacking events, or on detection based on third party services and reactive approaches that might take up to several hours. In this work, we present the results of a survey we conducted among 75 network operators to study: (a) the operators' awareness of BGP prefix hijacking attacks, (b) presently used defenses (if any) against BGP prefix hijacking, (c) the willingness to adopt new defense mechanisms, and (d) reasons that may hinder the deployment of BGP prefix hijacking defenses. We expect the findings of this survey to increase the understanding of existing BGP hijacking defenses and the needs of network operators, as well as contribute towards designing new defense mechanisms that satisfy the requirements of the operators.

==> questions_of_the_survey.tex <==
\blue{[I added the questions in the caption of the figures, so we can now remove this section --pavlos]}


%\subsection*{Information about the participants and their organizations}
{\large\textbf{Information about the participants and their organizations}}

\myitem{Question 1:} Which term(s) would best characterize your organization? (Fig.~\ref{fig:survey-q1})

\myitem{Question 2:} In which continent(s) does your company operate? (Fig.~\ref{fig:survey-q2})

\myitem{Question 3:} In which country(-ies) does your company operate? (optional) (Fig.~\ref{fig:survey-q3})

\myitem{Question 4:} What is your position in your company? (Fig.~\ref{fig:survey-q4})


%\subsection*{Knowledge and Experience with BGP Prefix Hijacking}
\vspace{\baselineskip}
\noindent
{\large\textbf{Knowledge and Experience with BGP Prefix Hijacking}}

\myitem{Question 5:} Do you know what BGP prefix hijacking is and how it can happen? (Fig.~\ref{fig:survey-q5})

\myitem{Question 6:} How concerned are you about BGP prefix hijacking incidents on the Internet? (Fig.~\ref{fig:survey-q6})

\myitem{Question 7:} Are you concerned that your network may be a victim of a BGP prefix hijacking incident in the future? (Fig.~\ref{fig:survey-q7})

\myitem{Question 8:} How severe do you consider the potential impact of a BGP prefix hijacking against your network? (Table~\ref{table:survey-q8})

\myitem{Question 9:} Has your organization been a victim of a BGP prefix hijacking incident in the past? (Fig.~\ref{fig:survey-q9})

\myitem{Question 10:} If your organization was a victim of a BGP prefix hijacking incident, for how long was your network affected? (optional) (Fig.~\ref{fig:survey-q10})

%\subsection*{Defenses against BGP Prefix Hijacking}
\vspace{\baselineskip}
\noindent
{\large\textbf{Defenses against BGP Prefix Hijacking}}

\myitem{Question 11:} Do you use RPKI in your network? (Fig.~\ref{fig:survey-q11})

\myitem{Question 12:} If no, what are the main reasons for not using RPKI? (optional) (Fig.~\ref{fig:survey-q12})

\myitem{Question 13:} Do you use in your network any other defense mechanisms (other than RPKI) that protect your/others' prefixes from BGP prefix hijacking? (Fig.~\ref{fig:survey-q13})

\myitem{Question 14:} If yes, what mechanisms do you use? Could you provide a brief description? (open question/answers - optional) (Fig.~\ref{fig:survey-q14})

\myitem{Question 15:} In your network, how would you learn about a hijacking incident against your prefix(es)? (Fig.~\ref{fig:survey-q15})

\myitem{Question 16:} If you use a local or third-party detection service or system, could you please give us more details about it? (open question/answers - optional) (Fig.~\ref{fig:survey-q16})

\myitem{Question 17:} How would you mitigate a hijack against your prefixes if you were notified about an on-going event? (Fig.~\ref{fig:survey-q17})

\myitem{Question 18:} Would you outsource functions relating to the detection and mitigation of prefix hijacking incidents to a third-party, if this helps your organization reduce its risks? (Fig.~\ref{fig:survey-q18})

\myitem{Question 19:} If no, what are the main factors that would affect your decision not to outsource prefix hijacking mitigation? (max 2 answers - optional) (Fig.~\ref{fig:survey-q19})

\myitem{Question 20:} Assuming you fully trust an outsourcing organization for prefix hijacking mitigation, what is the information/control (if any) you are still NOT willing to share/allow? (Fig.~\ref{fig:survey-q20})

\myitem{Question 21:} How important do you consider the following characteristics for the deployment of a new defense system in your network? (Fig.~\ref{fig:survey-q21} and Table~\ref{table:survey-q21})
